DynamicMind: A Tri-Mode Thinking System for Large Language Models

Modern large language models (LLMs) often struggle to dynamically adapt their reasoning depth to varying task complexities, leading to suboptimal performance or inefficient resource utilization. To address this, we introduce DynamicMind, a novel tri-mode thinking system. DynamicMind empowers LLMs to autonomously select between Fast, Normal, and Slow thinking modes for zero-shot question answering (ZSQA) tasks through cognitive-inspired prompt engineering. Our framework's core innovations include: (1) expanding the established dual-process framework of fast and slow thinking into a tri-mode thinking system involving a normal thinking mode to preserve the intrinsic capabilities of LLM; (2) proposing the Thinking Density metric, which aligns computational resource allocation with problem complexity; and (3) developing the Thinking Mode Capacity (TMC) dataset and a lightweight Mind Router to predict the optimal thinking mode. Extensive experiments across diverse mathematical, commonsense, and scientific QA benchmarks demonstrate that DynamicMind achieves superior ZSQA capabilities while establishing an effective trade-off between performance and computational efficiency.

==> latex/section/method_legacy.tex <==
\section{Methodology}
\label{methodology}
% % problem set
% % 性能测试
% % router


In this section, we introduce the proposed DynamicMind Framework. 



\subsection{Overview}
Figure \ref{fig:MD_framework} shows the DynamicMind framework, comprising the LLM Thinker and the Mind Router. Inspired by the Dual Process Theory of human cognition, the LLM Thinker operates in three modes: 1) \textbf{Normal Mode} represents the default reasoning paradigm without interference. 2) \textbf{Fast Mode} provides quick, intuitive, result-driven feedback, akin to System 1 in cognitive science. 3) \textbf{Slow Mode} involves extended CoT reasoning, reflecting System 2 with prolonged rationales and careful consideration. The Mind Router selects the optimal thinking mode based on the question's structure, and the LLM Thinker applies this mode for reasoning and inference. By leveraging these distinct modes, DynamicMind dynamically adjusts resource allocation, optimizing the model's reasoning approach for each task.





\subsection{LLM Thinker: Thinking as Human Systems}
In this section, we detailed to the LLM Thinker, incorporating with its three separate thinking mode designs.
\paragraph{Normal Mode}
In contrast to the dual-process theory of human cognition, we introduce the normal mode to preserve the inherent reasoning capabilities that LLMs acquire through their pre-training and post-training stages. 
It is also the common usage of LLMs where giving the questions to them without any restrictions of its thinking mode.
The reason of this decision is that most existing LLMs have been trained on data that partially contains CoT \cite{qwen2.5, dubey2024llama, deepseekai2024deepseekv3technicalreport}, enabling the models to possess certain logical reasoning abilities and decide when to use them. 
It is akin to a certain degree of integration between System 1 and System 2, preserving the model's own thinking abilities. 
% 补充一点缺点

\paragraph{Fast Mode}
We define the fast mode of LLM Thinker as it providing direct answers to given input questions without any additional content, such as analysis of the question, intermediate reasoning steps, or verification of the final answer. This mode directly leverages the LLM Thinker's knowledge learned during the pre-training and post-training phase. Many tasks can be successfully solved in this manner without the need for additional computation for intermediate steps \cite{radford2019language}. While fast thinking excels at quickly processing simple and familiar tasks with minimal computational requirements, it may produce incorrect answers or lack accuracy when faced with complex or ambiguous questions due to the lack of in-depth analysis and reasoning.

\paragraph{Slow Mode}
The Slow Mode requires the LLM Thinker to align with human System 2, which engaging in complex, meticulous, and rigorous logical thinking. For example, models like OpenAI O1 \cite{openai2024learning} and DeepSeek R1 \cite{deepseekai2025deepseekr1incentivizingreasoningcapability} incorporate various intermediate reasoning steps, allowing for a deeper analysis of the problem and a step-by-step conclusion. These models are able to handle complex problems, providing higher accuracy and reliability even in zero-shot condition. It can conduct thorough analysis and reasoning, making it suitable for tasks that demand careful consideration. However, the downside of slow mode is that it incurs higher computational costs and slower processing speeds. More critically, this mode is susceptible to overthinking phenomena, where excessive computational resources are allocated to straightforward problems without corresponding performance benefits \citep{chen2024not}.

% Specifically, the Normal Mode operates without any interference, representing the default reasoning paradigm. The Fast Mode requires the model to provide quick, intuitive, and result-driven feedback, omitting explanations and reasoning processes, corresponding to System 1 in cognitive science. In contrast, the Slow Mode compels the model to engage in extended CoT reasoning, incorporating prolonged reflection and careful consideration, mirroring System 2. 

%在这一节分别介绍三种模式。首先给出表格对比他们的特性，比如fast mode |思考快 | human system1 | average token on xx set|。
%然后列点1) Fast Mode (System 1)
%2) Medium Mode (System 2)
%3) Slow Mode (System 3)等分别介绍我们是怎么让他们和Human System对齐的 (Prompt)，实际对齐w效果如何 (Performance + token length，推理时间等等)

%注意，将你做实验，调prompt的方面的一些细节和思考写出来，以及这样做的优势，为什么当时选择这样做，(有哪些其他做法，为什么不这么做之类的,如果有的话） 核心是说明合理性

% 例如，无需训练，。。。




\subsection{Mind Router: Dynamic Routing on Thinking Systems}
It is essential to choose the appropriate thinking mode based on the specific requirements of the task at hand. But the key question in developing an optimal mind router lies in
\begin{itemize}
    \item[] \textit{How can we comprehensively understand the capabilities and efficiency of LLM Thinker's distinct reasoning modes across different tasks?}
\end{itemize}

To address this challenge, we design a probe-based method to evaluate the reasoning capabilities and efficiency of LLM Thinker's different thinking modes. Through this paradigm, we introduce the \textbf{ThinkMode Dataset}, the first-of-its-kind benchmark specifically designed to expose and analyze model thinking patterns – a significant contribution that enables unprecedented inspection of LLM cognition mechanisms.
%定义理想的controller 公式化描述总是最佳的
%Theorem 1: controller控制下的Reasoner总是比任何单一模式的reasoner都好


% To fully utilize the inherent fast and slow thinking capabilities of existing models, our Dynamic Mind (DM) framework endows the model's mind with $M = \{M_f, M_n, M_s\}$, representing Fast, Normal, and Slow thinking modes, as illustrated in Figure ~\ref{fig:MD framework}. We use zero-shot pass@k score $S_{k}$ and the number of generated tokens $N$ for a response to evaluate model's thinking quality and cognitive loads. We implement $M$ using the simplest method, which adjusting the prompt for different thinking modes. It's worth noting that DM can accommodate any methods that can control a model's thinking modes.

\paragraph{Thinking System Probing}
\label{probing}

Our methodology employs two orthogonal metrics: (1) \textit{thinking competence}, measured by the accuracy of multiple thinking attempts for each problem under specific modes, and (2) \textit{thinking efficiency}, quantified through the average number of tokens generated during the thinking process.

We adopt a hierarchical evaluation framework that prioritizes thinking competence over efficiency, reflecting the practical prioritization of solution quality in most real-world LLM applications. This two-stage assessment strategy ensures that efficiency comparisons are only conducted between modes demonstrating equivalent competence levels.
Our investigates two representative task categories:
\begin{itemize}
    \item Commonsense question answering tasks demanding automatic retrieval of established knowledge, optimally suited for fast mode
    \item Mathematical problems  demanding formal logic execution, inherently favoring deliberative slow mode
    
\end{itemize}

% 数据集分布，讨论确实需要Mind Router
Figure 2 presents a comprehensive comparison of the three reasoning modes across both competence and efficiency dimensions. The results reveal significant performance variations that inform optimal mode selection strategies based on task requirements and operational constraints.

\paragraph{Mind Router Training}
\section{Methodology}
\label{methodology}
% % problem set
% % 性能测试
% % router


In this section, we introduce the proposed DynamicMind Framework. 



\subsection{Overview}
Figure \ref{fig:MD_framework} shows the DynamicMind framework, comprising the LLM Thinker and the Mind Router. Inspired by the Dual Process Theory of human cognition, the LLM Thinker operates in three modes: 1) \textbf{Normal Mode} represents the default reasoning paradigm without interference. 2) \textbf{Fast Mode} provides quick, intuitive, result-driven feedback, akin to System 1 in cognitive science. 3) \textbf{Slow Mode} involves extended CoT reasoning, reflecting System 2 with prolonged rationales and careful consideration. The Mind Router selects the optimal thinking mode based on the question's structure, and the LLM Thinker applies this mode for reasoning and inference. By leveraging these distinct modes, DynamicMind dynamically adjusts resource allocation, optimizing the model's reasoning approach for each task.





\subsection{LLM Thinker: Thinking as Human Systems}
In this section, we detailed to the LLM Thinker, incorporating with its three separate thinking mode designs.
\paragraph{Normal Mode}
In contrast to the dual-process theory of human cognition, we introduce the normal mode to preserve the inherent reasoning capabilities that LLMs acquire through their pre-training and post-training stages. 
It is also the common usage of LLMs where giving the questions to them without any restrictions of its thinking mode.
The reason of this decision is that most existing LLMs have been trained on data that partially contains CoT \cite{qwen2.5, dubey2024llama, deepseekai2024deepseekv3technicalreport}, enabling the models to possess certain logical reasoning abilities and decide when to use them. 
It is akin to a certain degree of integration between System 1 and System 2, preserving the model's own thinking abilities. 
% 补充一点缺点

\paragraph{Fast Mode}
We define the fast mode of LLM Thinker as it providing direct answers to given input questions without any additional content, such as analysis of the question, intermediate reasoning steps, or verification of the final answer. This mode directly leverages the LLM Thinker's knowledge learned during the pre-training and post-training phase. Many tasks can be successfully solved in this manner without the need for additional computation for intermediate steps \cite{radford2019language}. While fast thinking excels at quickly processing simple and familiar tasks with minimal computational requirements, it may produce incorrect answers or lack accuracy when faced with complex or ambiguous questions due to the lack of in-depth analysis and reasoning.

\paragraph{Slow Mode}
The Slow Mode requires the LLM Thinker to align with human System 2, which engaging in complex, meticulous, and rigorous logical thinking. For example, models like OpenAI O1 \cite{openai2024learning} and DeepSeek R1 \cite{deepseekai2025deepseekr1incentivizingreasoningcapability} incorporate various intermediate reasoning steps, allowing for a deeper analysis of the problem and a step-by-step conclusion. These models are able to handle complex problems, providing higher accuracy and reliability even in zero-shot condition. It can conduct thorough analysis and reasoning, making it suitable for tasks that demand careful consideration. However, the downside of slow mode is that it incurs higher computational costs and slower processing speeds. More critically, this mode is susceptible to overthinking phenomena, where excessive computational resources are allocated to straightforward problems without corresponding performance benefits \citep{chen2024not}.

% Specifically, the Normal Mode operates without any interference, representing the default reasoning paradigm. The Fast Mode requires the model to provide quick, intuitive, and result-driven feedback, omitting explanations and reasoning processes, corresponding to System 1 in cognitive science. In contrast, the Slow Mode compels the model to engage in extended CoT reasoning, incorporating prolonged reflection and careful consideration, mirroring System 2. 

%在这一节分别介绍三种模式。首先给出表格对比他们的特性，比如fast mode |思考快 | human system1 | average token on xx set|。
%然后列点1) Fast Mode (System 1)
%2) Medium Mode (System 2)
%3) Slow Mode (System 3)等分别介绍我们是怎么让他们和Human System对齐的 (Prompt)，实际对齐w效果如何 (Performance + token length，推理时间等等)

%注意，将你做实验，调prompt的方面的一些细节和思考写出来，以及这样做的优势，为什么当时选择这样做，(有哪些其他做法，为什么不这么做之类的,如果有的话） 核心是说明合理性

% 例如，无需训练，。。。




\subsection{Mind Router: Dynamic Routing on Thinking Systems}
It is essential to choose the appropriate thinking mode based on the specific requirements of the task at hand. But the key question in developing an optimal mind router lies in
\begin{itemize}
    \item[] \textit{How can we comprehensively understand the capabilities and efficiency of LLM Thinker's distinct reasoning modes across different tasks?}
\end{itemize}

To address this challenge, we design a probe-based method to evaluate the reasoning capabilities and efficiency of LLM Thinker's different thinking modes. Through this paradigm, we introduce the \textbf{ThinkMode Dataset}, the first-of-its-kind benchmark specifically designed to expose and analyze model thinking patterns – a significant contribution that enables unprecedented inspection of LLM cognition mechanisms.
%定义理想的controller 公式化描述总是最佳的
%Theorem 1: controller控制下的Reasoner总是比任何单一模式的reasoner都好


% To fully utilize the inherent fast and slow thinking capabilities of existing models, our Dynamic Mind (DM) framework endows the model's mind with $M = \{M_f, M_n, M_s\}$, representing Fast, Normal, and Slow thinking modes, as illustrated in Figure ~\ref{fig:MD framework}. We use zero-shot pass@k score $S_{k}$ and the number of generated tokens $N$ for a response to evaluate model's thinking quality and cognitive loads. We implement $M$ using the simplest method, which adjusting the prompt for different thinking modes. It's worth noting that DM can accommodate any methods that can control a model's thinking modes.

\paragraph{Thinking System Probing}
\label{probing}

Our methodology employs two orthogonal metrics: (1) \textit{thinking competence}, measured by the accuracy of multiple thinking attempts for each problem under specific modes, and (2) \textit{thinking efficiency}, quantified through the average number of tokens generated during the thinking process.

We adopt a hierarchical evaluation framework that prioritizes thinking competence over efficiency, reflecting the practical prioritization of solution quality in most real-world LLM applications. This two-stage assessment strategy ensures that efficiency comparisons are only conducted between modes demonstrating equivalent competence levels.
Our investigates two representative task categories:
\begin{itemize}
    \item Commonsense question answering tasks demanding automatic retrieval of established knowledge, optimally suited for fast mode
    \item Mathematical problems  demanding formal logic execution, inherently favoring deliberative slow mode
    
\end{itemize}

% 数据集分布，讨论确实需要Mind Router
Figure 2 presents a comprehensive comparison of the three reasoning modes across both competence and efficiency dimensions. The results reveal significant performance variations that inform optimal mode selection strategies based on task requirements and operational constraints.

\paragraph{Mind Router Training}
\section{Methodology}
\label{methodology}
% % problem set
% % 性能测试
% % router


In this section, we introduce the proposed DynamicMind Framework. 



\subsection{Overview}
Figure \ref{fig:MD_framework} shows the DynamicMind framework, comprising the LLM Thinker and the Mind Router. Inspired by the Dual Process Theory of human cognition, the LLM Thinker operates in three modes: 1) \textbf{Normal Mode} represents the default reasoning paradigm without interference. 2) \textbf{Fast Mode} provides quick, intuitive, result-driven feedback, akin to System 1 in cognitive science. 3) \textbf{Slow Mode} involves extended CoT reasoning, reflecting System 2 with prolonged rationales and careful consideration. The Mind Router selects the optimal thinking mode based on the question's structure, and the LLM Thinker applies this mode for reasoning and inference. By leveraging these distinct modes, DynamicMind dynamically adjusts resource allocation, optimizing the model's reasoning approach for each task.





\subsection{LLM Thinker: Thinking as Human Systems}
In this section, we detailed to the LLM Thinker, incorporating with its three separate thinking mode designs.
\paragraph{Normal Mode}
In contrast to the dual-process theory of human cognition, we introduce the normal mode to preserve the inherent reasoning capabilities that LLMs acquire through their pre-training and post-training stages. 
It is also the common usage of LLMs where giving the questions to them without any restrictions of its thinking mode.
The reason of this decision is that most existing LLMs have been trained on data that partially contains CoT \cite{qwen2.5, dubey2024llama, deepseekai2024deepseekv3technicalreport}, enabling the models to possess certain logical reasoning abilities and decide when to use them. 
It is akin to a certain degree of integration between System 1 and System 2, preserving the model's own thinking abilities. 
% 补充一点缺点

\paragraph{Fast Mode}
We define the fast mode of LLM Thinker as it providing direct answers to given input questions without any additional content, such as analysis of the question, intermediate reasoning steps, or verification of the final answer. This mode directly leverages the LLM Thinker's knowledge learned during the pre-training and post-training phase. Many tasks can be successfully solved in this manner without the need for additional computation for intermediate steps \cite{radford2019language}. While fast thinking excels at quickly processing simple and familiar tasks with minimal computational requirements, it may produce incorrect answers or lack accuracy when faced with complex or ambiguous questions due to the lack of in-depth analysis and reasoning.

\paragraph{Slow Mode}
The Slow Mode requires the LLM Thinker to align with human System 2, which engaging in complex, meticulous, and rigorous logical thinking. For example, models like OpenAI O1 \cite{openai2024learning} and DeepSeek R1 \cite{deepseekai2025deepseekr1incentivizingreasoningcapability} incorporate various intermediate reasoning steps, allowing for a deeper analysis of the problem and a step-by-step conclusion. These models are able to handle complex problems, providing higher accuracy and reliability even in zero-shot condition. It can conduct thorough analysis and reasoning, making it suitable for tasks that demand careful consideration. However, the downside of slow mode is that it incurs higher computational costs and slower processing speeds. More critically, this mode is susceptible to overthinking phenomena, where excessive computational resources are allocated to straightforward problems without corresponding performance benefits \citep{chen2024not}.

% Specifically, the Normal Mode operates without any interference, representing the default reasoning paradigm. The Fast Mode requires the model to provide quick, intuitive, and result-driven feedback, omitting explanations and reasoning processes, corresponding to System 1 in cognitive science. In contrast, the Slow Mode compels the model to engage in extended CoT reasoning, incorporating prolonged reflection and careful consideration, mirroring System 2. 

%在这一节分别介绍三种模式。首先给出表格对比他们的特性，比如fast mode |思考快 | human system1 | average token on xx set|。
%然后列点1) Fast Mode (System 1)
%2) Medium Mode (System 2)
%3) Slow Mode (System 3)等分别介绍我们是怎么让他们和Human System对齐的 (Prompt)，实际对齐w效果如何 (Performance + token length，推理时间等等)

%注意，将你做实验，调prompt的方面的一些细节和思考写出来，以及这样做的优势，为什么当时选择这样做，(有哪些其他做法，为什么不这么做之类的,如果有的话） 核心是说明合理性

% 例如，无需训练，。。。




\subsection{Mind Router: Dynamic Routing on Thinking Systems}
It is essential to choose the appropriate thinking mode based on the specific requirements of the task at hand. But the key question in developing an optimal mind router lies in
\begin{itemize}
    \item[] \textit{How can we comprehensively understand the capabilities and efficiency of LLM Thinker's distinct reasoning modes across different tasks?}
\end{itemize}

To address this challenge, we design a probe-based method to evaluate the reasoning capabilities and efficiency of LLM Thinker's different thinking modes. Through this paradigm, we introduce the \textbf{ThinkMode Dataset}, the first-of-its-kind benchmark specifically designed to expose and analyze model thinking patterns – a significant contribution that enables unprecedented inspection of LLM cognition mechanisms.
%定义理想的controller 公式化描述总是最佳的
%Theorem 1: controller控制下的Reasoner总是比任何单一模式的reasoner都好


% To fully utilize the inherent fast and slow thinking capabilities of existing models, our Dynamic Mind (DM) framework endows the model's mind with $M = \{M_f, M_n, M_s\}$, representing Fast, Normal, and Slow thinking modes, as illustrated in Figure ~\ref{fig:MD framework}. We use zero-shot pass@k score $S_{k}$ and the number of generated tokens $N$ for a response to evaluate model's thinking quality and cognitive loads. We implement $M$ using the simplest method, which adjusting the prompt for different thinking modes. It's worth noting that DM can accommodate any methods that can control a model's thinking modes.

\paragraph{Thinking System Probing}
\label{probing}

Our methodology employs two orthogonal metrics: (1) \textit{thinking competence}, measured by the accuracy of multiple thinking attempts for each problem under specific modes, and (2) \textit{thinking efficiency}, quantified through the average number of tokens generated during the thinking process.

We adopt a hierarchical evaluation framework that prioritizes thinking competence over efficiency, reflecting the practical prioritization of solution quality in most real-world LLM applications. This two-stage assessment strategy ensures that efficiency comparisons are only conducted between modes demonstrating equivalent competence levels.
Our investigates two representative task categories:
\begin{itemize}
    \item Commonsense question answering tasks demanding automatic retrieval of established knowledge, optimally suited for fast mode
    \item Mathematical problems  demanding formal logic execution, inherently favoring deliberative slow mode
    
\end{itemize}

% 数据集分布，讨论确实需要Mind Router
Figure 2 presents a comprehensive comparison of the three reasoning modes across both competence and efficiency dimensions. The results reveal significant performance variations that inform optimal mode selection strategies based on task requirements and operational constraints.

\paragraph{Mind Router Training}


==> latex/tables/datasets_statistic.tex <==
\begin{table}[h!t]
    \centering
   % \vskip -0.13in
    \caption{{The dataset statistics.}} 

    \label{tab:datasets_statistics}
%    \vskip 0.08in
    \setlength{\tabcolsep}{3pt}
    \resizebox{0.4\linewidth}{!}{
    \begin{tabular}{lcccc}
    \toprule
    % \cmidrule(lr){3-6}
    % \cmidrule(lr){8-11}
    \textbf{Datasets} & & Training Set Size &  & Test Set Size  \\
    % \midrule
    \midrule
    \multicolumn{5}{c}{\textit{In-domain Datasets}} \\
    \midrule
    Math & & & & 5000\\
    GSM8K & & & & 1319\\
    BoolQ & & & & 3270\\
    PIQA & & & & 1838\\
    SIQA & & & & 1954\\ 
    HellaSwag & & & & 10042\\
    WinoGrande & & & & 1267\\
    ARC-e & & & & 2376\\
    ARC-c & & & & 1172\\
    OBQA & & & & 500\\
    \midrule
    MMLU \\
    jurisprudence nutrition management marketing formal_logic high_school_european_history
    \ \ \ \ \ \ clinical knowledge \\
    \ \ \ \ \ \ college biology \\
    \ \ \ \ \ \ college medicine \\
    \ \ \ \ \ \ college computer science \\
    \ \ \ \ \ \ sociology \\
    \ \ \ \ \ \ econometrics \\
    \ \ \ \ \ \ professional psychology \\
    \ \ \ \ \ \ professional law \\
    \ \ \ \ \ \ professional medicine \\
    \ \ \ \ \ \ test \\
    \ \ \ \ \ \ test \\
    ScienceQA \\
    \ \ \ \ \ \ test \\
    \bottomrule
\end{tabular}
}
\vspace{-5pt}
\end{table}

==> latex/tables/router_distributions.tex <==
\begin{table*}[t]
    \centering
%    \vskip -0.13in
    \caption{\footnotesize{.}} 
%    \vskip 0.08in
    \setlength{\tabcolsep}{6pt}
    \resizebox{0.7\linewidth}{!}{
    \begin{tabular}{lccccccccccccccc}
    \toprule
    % \cmidrule(lr){3-6}
    % \cmidrule(lr){8-11}
    \textbf{MindRouter} & \multicolumn{3}{c}{Math} & \multicolumn{3}{c}{CommonsenseQA} & \multicolumn{3}{c}{MMLU} & \multicolumn{3}{c}{ScienceQA} & \multicolumn{3}{c}{\textbf{Overall}} \\
     & F & N & S & F & N & S & F & N & S & F & N & S & F & N & S \\
    \midrule
    Llama's & 9.16 & 79.22 & 11.62 & 74.77 & 0.07 & 25.16 & 33.96 & 61.04 & 5.00 & 81.79 & 15.00 & 3.21 & 58.49 & 22.93 & 18.58 \\
    Qwen's & 3.28 & 96.11 & 0.62 & 89.94 & 2.33 & 7.73 & 24.43 & 77.56 & 0.09 & 39.66 & 59.39 & 0.95 & 62.60 & 32.40 & 5.00 \\
    

    \bottomrule
\end{tabular}
}

\label{tab:transfer}
\end{table*}
